MIRAGE: Mitigating Conflict-Based Cache Attacks with a Practical Fully-Associative Design

Shared processor caches are vulnerable to conflict-based side-channel attacks, where an attacker can monitor access patterns of a victim by evicting victim cache lines using cache-set conflicts. Recent mitigations propose randomized mapping of addresses to cache lines to obfuscate the locations of set-conflicts. However, these are vulnerable to new attacks that discover conflicting sets of addresses despite such mitigations, because these designs select eviction-candidates from a small set of conflicting lines. This paper presents Mirage, a practical design for a fully associative cache, wherein eviction candidates are selected randomly from all lines resident in the cache, to be immune to set-conflicts. A key challenge for enabling such designs in large shared caches (containing tens of thousands of cache lines) is the complexity of cache-lookup, as a naive design can require searching through all the resident lines. Mirage achieves full-associativity while retaining practical set-associative lookups by decoupling placement and replacement, using pointer-based indirection from tag-store to data-store to allow a newly installed address to globally evict the data of any random resident line. To eliminate set-conflicts, Mirage provisions extra invalid tags in a skewed-associative tag-store design where lines can be installed without set-conflict, along with a load-aware skew-selection policy that guarantees the availability of sets with invalid tags. Our analysis shows Mirage provides the global eviction property of a fully-associative cache throughout system lifetime (violations of full-associativity, i.e. set-conflicts, occur less than once in 10^4 to 10^17 years), thus offering a principled defense against any eviction-set discovery and any potential conflict based attacks. Mirage incurs limited slowdown (2%) and 17-20% extra storage compared to a non-secure cache.

==> sigproc_long.tex <==

@TECHREPORT{Bernstein,
    author = {Daniel J. Bernstein},
    title = {Cache-timing attacks on AES},
    institution = {},
    year = {2005}
}

@inproceedings{GetOffMyCloud,
author = {Ristenpart, Thomas and Tromer, Eran and Shacham, Hovav and Savage, Stefan},
title = {Hey, You, Get off of My Cloud: Exploring Information Leakage in Third-Party Compute Clouds},
year = {2009},
booktitle = {Proceedings of the 16th ACM Conference on Computer and Communications Security},
series = {CCS ’09}
}
  



@inproceedings{PrimeProbe,
 author = {Osvik, Dag Arne and Shamir, Adi and Tromer, Eran},
 title = {Cache Attacks and Countermeasures: The Case of AES},
 booktitle = {Proceedings of the 2006 The Cryptographers' Track at the RSA Conference on Topics in Cryptology},
 series = {CT-RSA'06},
 year = {2006}
} 


@INPROCEEDINGS{isca19:SkewedCEASER, 
	author={Moinuddin K. Qureshi}, 
	booktitle={Proceedings of the 46th International Symposium on Computer Architecture (ISCA)},
	title={New attacks and defense for encrypted-address cache}, 
	year={2019}
    }

@INPROCEEDINGS{micro18:CEASER, 
	author={Moinuddin K. Qureshi}, 
	booktitle={Proceedings of the 51st Annual IEEE/ACM International Symposium on Microarchitecture}, 
	title={ {CEASER}: Mitigating Conflict-Based Cache Attacks via Dynamically Encrypted Address}, 
	year={2018},
    }

@inproceedings {ScatterCache,
author = {Mario Werner and Thomas Unterluggauer and Lukas Giner and Michael Schwarz and Daniel Gruss and Stefan Mangard},
title = {ScatterCache: Thwarting Cache Attacks via Cache Set Randomization},
booktitle = {USENIX Security},
year = {2019}
}

@inproceedings{seznec_skew,
author = {Seznec, Andr\'{e}},
title = {A Case for Two-Way Skewed-Associative Caches},
year = {1993},
booktitle = {Proceedings of the 20th Annual International Symposium on Computer Architecture},
series = {ISCA ’93}
}

@inproceedings{sp15:LLCAttacksPractical,
  title={Last-level cache side-channel attacks are practical},
  author={Liu, Fangfei and Yarom, Yuval and Ge, Qian and Heiser, Gernot and Lee, Ruby B},
  booktitle={Security and Privacy (SP), 2015 IEEE Symposium on},
  pages={605--622},
  year={2015},
  organization={IEEE}
}

@inproceedings{sp19:FastEvictionSets,
  title={Theory and practice of finding eviction sets},
  author={Vila, Pepe and K{\"o}pf, Boris and Morales, Jos{\'e} F},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={39--54},
  year={2019},
  organization={IEEE}
}

@article{KULeuven:ProbabilisticEvictionSets,
  title={Advanced profiling for probabilistic Prime+ Probe attacks and covert channels in ScatterCache},
  author={Purnal, Antoon and Verbauwhede, Ingrid},
  journal={arXiv preprint arXiv:1908.03383},
  year={2019}
}

@inproceedings{SP21:SystematicRandCaches,
  title={Systematic Analysis of Randomization-based Protected Cache Architectures},
  author={Purnal, Antoon and Giner, Lukas and Gruss, Daniel and Verbauwhede, Ingrid},
  booktitle={42th IEEE Symposium on Security and Privacy},
  year={2020}
}

@article{BalancedAllocations,
  title={Balanced allocations},
  author={Azar, Yossi and Broder, Andrei Z and Karlin, Anna R and Upfal, Eli},
  journal={SIAM journal on computing},
  volume={29},
  number={1},
  pages={180--200},
  year={1999},
  publisher={SIAM}
}

@article{Powerof2ChoicesSurvey,
  title={The power of two random choices: A survey of techniques and results},
  author={Richa, Andrea W and Mitzenmacher, M and Sitaraman, R},
  journal={Combinatorial Optimization},
  volume={9},
  pages={255--304},
  year={2001},
  publisher={Springer}
}

@article{LoadBalancing:AlwaysGoLeft,
  title={How asymmetry helps load balancing},
  author={V{\"o}cking, Berthold},
  journal={Journal of the ACM (JACM)},
  volume={50},
  number={4},
  pages={568--589},
  year={2003},
  publisher={ACM New York, NY, USA}
}


@INPROCEEDINGS{RandomFill, 
author={F. Liu and R. B. Lee}, 
booktitle={2014 47th Annual IEEE/ACM International Symposium on Microarchitecture}, 
title={Random Fill Cache Architecture}, 
year={2014}, 
volume={}, 
number={}, 
pages={203-215}, 
keywords={cache storage;cryptography;memory architecture;cache designs;cache side-channel attacks;confidentiality breaches;configurable neighborhood window;contention based attacks;encryption keys;fake services;fundamental demand fetch policy;impersonation attacks;information-theoretic security;random fill cache architecture;reuse based attacks;Computer architecture;Encryption;Hardware;Timing;cache;cache collision attacks;computer architecture;secure caches;security;side channel attacks}, 
doi={10.1109/MICRO.2014.28}, 
ISSN={1072-4451}, 
month={Dec},}


@inproceedings{CacheCollisionAttacks,
  title={Cache-collision timing attacks against AES},
  author={Bonneau, Joseph and Mironov, Ilya},
  booktitle={International Workshop on Cryptographic Hardware and Embedded Systems},
  pages={201--215},
  year={2006},
  organization={Springer}
}


@inproceedings{FlushFlush,
  title={Flush+ Flush: a fast and stealthy cache attack},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Wagner, Klaus and Mangard, Stefan},
  booktitle={DIMVA},
  year={2016},
}


@inproceedings{yaromFlushReload,
  title={FLUSH+ RELOAD: A High Resolution, Low Noise, L3 Cache Side-Channel Attack.},
  author={Yarom, Yuval and Falkner, Katrina},
  booktitle={USENIX Security},
  year={2014}
} 


@inproceedings{yao:coherence,
  title={Are Coherence Protocol States Vulnerable to Information Leakage?},
  author={Yao, Fan and Doroslovacki, Milos and Venkataramani, Guru},
  booktitle={HPCA},
  year={2018},
}

@INPROCEEDINGS{sharp,
author = {M. Yan and B. Gopireddy and T. Shull and J. Torrellas},
booktitle = {ISCA},
title = {Secure hierarchy-aware cache replacement policy (SHARP): Defending against cache-based side channel attacks},
year = {2017},
}

@INPROCEEDINGS{DAWG, 
  author={Kiriansky, Vladimir and Lebedev, Ilia and Amarasinghe, Saman and Devadas, Srinivas and Emer, Joel},
  title={{DAWG: A Defense Against Cache Timing Attacks in Speculative Execution Processors}},
  booktitle={MICRO}, 
  year={2018}}


@inproceedings{NewCache,
 author = {Zhenghong Wang and Lee, Ruby B.},
 title = {A Novel Cache Architecture with Enhanced Performance and Security},
 booktitle = {International Symposium on Microarchitecture},
 series = {MICRO},
 year = {2008},
} 

@inproceedings{RPCache,
  title={New cache designs for thwarting software cache-based side channel attacks},
  author={Wang, Zhenghong and Lee, Ruby B},
  booktitle={Proceedings of the 34th annual international symposium on Computer architecture},
  pages={494--505},
  year={2007}
}

@inproceedings{Vway,
  title={The V-Way cache: demand-based associativity via global replacement},
  author={Qureshi, Moinuddin K and Thompson, David and Patt, Yale N},
  booktitle={32nd International Symposium on Computer Architecture (ISCA'05)},
  pages={544--555},
  year={2005},
  organization={IEEE}
}

@article{RRIP,
  title={High performance cache replacement using re-reference interval prediction (RRIP)},
  author={Jaleel, Aamer and Theobald, Kevin B and Steely Jr, Simon C and Emer, Joel},
  journal={ACM SIGARCH Computer Architecture News},
  volume={38},
  number={3},
  pages={60--71},
  year={2010},
  publisher={ACM New York, NY, USA}
}

@inproceedings{HPCA20:LRUAttack,
  title={Leaking Information Through Cache LRU States},
  author={Xiong, Wenjie and Szefer, Jakub},
  booktitle={HPCA},
  year={2020},
}

@inproceedings{Usenix2020:RRIPAttack,
  title={Reload+ refresh: Abusing cache replacement policies to perform stealthy cache attacks},
  author={Briongos, Samira and Malag{\'o}n, Pedro and Moya, Jos{\'e} M and Eisenbarth, Thomas},
  booktitle={Usenix Security},
  year={2020}
}

@inproceedings{PhantomCache,
  title={PhantomCache: Obfuscating Cache Conflicts with Localized Randomization},
  author={Tan, Qinhan and Zeng, Zhihua and Bu, Kai and Ren, Kui},
  booktitle={NDSS},
  year={2020}
}

@inproceedings{MI6,
  title={MI6: Secure enclaves in a speculative out-of-order processor},
  author={Bourgeat, Thomas and Lebedev, Ilia and Wright, Andrew and Zhang, Sizhuo and Devadas, Srinivas},
  booktitle={Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
  year={2019}
}

@inproceedings{PageColoring,
  title={Resource management for isolation enhanced cloud services},
  author={Raj, Himanshu and Nathuji, Ripal and Singh, Abhishek and England, Paul},
  booktitle={Proceedings of the 2009 ACM workshop on Cloud computing security},
  year={2009}
}

@inproceedings{StealthMem,
  title={{STEALTHMEM}: System-Level Protection Against Cache-Based Side Channel Attacks in the Cloud},
  author={Kim, Taesoo and Peinado, Marcus and Mainar-Ruiz, Gloria},
  booktitle={{21st USENIX Security Symposium (USENIX Security 12)}},
  year={2012}
}

@inproceedings{Catalyst,
  title={Catalyst: Defeating last-level cache side channel attacks in cloud computing},
  author={Liu, Fangfei and Ge, Qian and Yarom, Yuval and Mckeen, Frank and Rozas, Carlos and Heiser, Gernot and Lee, Ruby B},
  booktitle={2016 IEEE international symposium on high performance computer architecture (HPCA)},
  pages={406--418},
  year={2016},
  organization={IEEE}
}

@inproceedings{PrefetcherCommonSense,
  title={Fooling the Sense of Cross-core Last-level Cache Eviction based Attacker by Prefetching Common Sense},
  author={Panda, Biswabandan},
  booktitle={2019 28th International Conference on Parallel Architectures and Compilation Techniques (PACT)},
  pages={138--150},
  year={2019},
  organization={IEEE}
}

@inproceedings{Cyclone,
  title={Cyclone: Detecting Contention-Based Cache Information Leaks Through Cyclic Interference},
  author={Harris, Austin and Wei, Shijia and Sahu, Prateek and Kumar, Pranav and Austin, Todd and Tiwari, Mohit},
  booktitle={Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={57--72},
  year={2019}
}

@inproceedings{CCHunter,
  title={Cc-hunter: Uncovering covert timing channels on shared processor hardware},
  author={Chen, Jie and Venkataramani, Guru},
  booktitle={2014 47th Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={216--228},
  year={2014},
  organization={IEEE}
}

@article{MitzenmacherThesis,
  title={The power of two choices in randomized load balancing},
  author={Mitzenmacher, Michael},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={12},
  number={10},
  pages={1094--1104},
  year={2001},
  publisher={IEEE}
}

@inproceedings{LoadBalancingHashtables,
  title={A scheme for load balancing in heterogenous distributed hash tables},
  author={Giakkoupis, George and Hadzilacos, Vassos},
  booktitle={Proceedings of the twenty-fourth annual ACM symposium on Principles of distributed computing},
  pages={302--311},
  year={2005}
}


@online{DanLuuBlog,
  author = {Luu, Dan},
  title = {Caches: LRU v. Random},
  howpublished={\url{https://danluu.com/2choices-eviction/}}
}

@online{IBMPower9,
    author = {WikiChip},
    title = {{POWER9 - Microarchitectures - IBM}},
    howpublished={\url{https://en.wikichip.org/wiki/ibm/microarchitectures/power9}},
}

@article{cacti6.0,
  title={CACTI 6.0: A tool to model large caches},
  author={Muralimanohar, Naveen and Balasubramonian, Rajeev and Jouppi, Norman P},
  journal={HP laboratories},
  volume={27},
  pages={28},
  year={2009}
}


@online{Qameleon,
  author = {Avanzi, Roberto and Banik, Subhadeep and Bogdanov, Andrey and Dunkelman, Orr and Huan, Senyang and Regazzon, Francesco },
  title = {Qameleon v1.0 - A Submission to the NIST Lightweight Cryptography Standardization  Process},
  howpublished={\url{https://csrc.nist.gov/CSRC/media/Projects/Lightweight-Cryptography/documents/round-1/spec-doc/qameleon-spec.pdf/}}
}

@article{qarma64,
  title={The QARMA block cipher family. Almost MDS matrices over rings with zero divisors, nearly symmetric even-mansour constructions with non-involutory central rounds, and search heuristics for low-latency s-boxes},
  author={Avanzi, Roberto},
  journal={IACR Transactions on Symmetric Cryptology},
  pages={4--44},
  year={2017}
}

@inproceedings{cuckoo_hashing,
  title={Cuckoo hashing},
  author={Pagh, Rasmus and Rodler, Flemming Friche},
  booktitle={European Symposium on Algorithms},
  pages={121--133},
  year={2001},
  organization={Springer}
}

@inproceedings{dram_access_energy,
  title={Understanding the energy consumption of dynamic random access memories},
  author={Vogelsang, Thomas},
  booktitle={2010 43rd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={363--374},
  year={2010},
  organization={IEEE}
}

@inproceedings{zcache,
  title={The ZCache: Decoupling ways and associativity},
  author={Sanchez, Daniel and Kozyrakis, Christos},
  booktitle={2010 43rd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={187--198},
  year={2010},
  organization={IEEE}
}

@inproceedings{cuckooDirectory,
  title={Cuckoo directory: A scalable directory for many-core systems},
  author={Ferdman, Michael and Lotfi-Kamran, Pejman and Balet, Ken and Falsafi, Babak},
  booktitle={2011 IEEE 17th International Symposium on High Performance Computer Architecture},
  pages={169--180},
  year={2011},
  organization={IEEE}
}

@inproceedings{iic,
  title={A fully associative software-managed cache design},
  author={Hallnor, Erik G and Reinhardt, Steven K},
  booktitle={Proceedings of 27th International Symposium on Computer Architecture (IEEE Cat. No. RS00201)},
  pages={107--116},
  year={2000},
  organization={IEEE}
}

@inproceedings{DirectoryAttacks,
  title={Attack directories, not caches: Side channel attacks in a non-inclusive world},
  author={Yan, Mengjia and Sprabery, Read and Gopireddy, Bhargava and Fletcher, Christopher and Campbell, Roy and Torrellas, Josep},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={888--904},
  year={2019},
  organization={IEEE}
}

@inproceedings{isca19:secdir,
  title={SecDir: a secure directory to defeat directory side-channel attacks},
  author={Yan, Mengjia and Wen, Jen-Yang and Fletcher, Christopher W and Torrellas, Josep},
  booktitle={Proceedings of the 46th International Symposium on Computer Architecture},
  pages={332--345},
  year={2019}
}

@INBOOK{birthdeath,
 author = {David Lilja},
 title = {Measuring Computer Performance},
 publisher = "Cambridge University Press",
 year      =  2000,
 pages = {228-229},
}

@inproceedings{CacheTelepathy,
  title={Cache telepathy: Leveraging shared resource attacks to learn DNN architectures},
  author={Yan, Mengjia and Fletcher, Christopher and Torrellas, Josep},
   booktitle={{29th USENIX Security Symposium (USENIX Security 20)}},
  year={2020}
}


@inproceedings{Netspectre,
  title={{Netspectre: Read arbitrary memory over network}},
  author={Schwarz, Michael and Schwarzl, Martin and Lipp, Moritz and Masters, Jon and Gruss, Daniel},
  booktitle={European Symposium on Research in Computer Security},
  pages={279--299},
  year={2019}
}

@inproceedings{Hybcache,
  title={HybCache: Hybrid Side-Channel-Resilient Caches for Trusted Execution Environments},
  author={Dessouky, Ghada and Frassetto, Tommaso and Sadeghi, Ahmad-Reza},
  booktitle={29th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 20)},
  year={2020}
}

@inproceedings{Cloak,
  title={Strong and efficient cache side-channel protection using hardware transactional memory},
  author={Gruss, Daniel and Lettner, Julian and Schuster, Felix and Ohrimenko, Olya and Haller, Istvan and Costa, Manuel},
  booktitle={26th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 17)},
  pages={217--233},
  year={2017}
}

%@inproceedings{CacheBar,
%  title={A software approach to defeating side channels in last-level caches},
%  author={Zhou, Ziqiao and Reiter, Michael K and Zhang, Yinqian},
%  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
%  pages={871--882},
%  year={2016}
%}


@inproceedings{CacheBar,
  title={A software approach to defeating side channels in last-level caches},
  author={Zhou, Ziqiao and Reiter, Michael K and Zhang, Yinqian},
  booktitle={CCS 2016},
  year={2016}
}

@inproceedings{InvalidateTransfer,
  title={Cross processor cache attacks},
  author={Irazoqui, Gorka and Eisenbarth, Thomas and Sunar, Berk},
  booktitle={Proceedings of the 11th ACM on Asia conference on computer and communications security},
  pages={353--364},
  year={2016}
}

@inproceedings{FlushPrefetch,
  title={Prefetch side-channel attacks: Bypassing SMAP and kernel ASLR},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Fogh, Anders and Lipp, Moritz and Mangard, Stefan},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={368--379},
  year={2016}
}

@inproceedings{EvictReload,
  title={Cache template attacks: Automating attacks on inclusive last-level caches},
  author={Gruss, Daniel and Spreitzer, Raphael and Mangard, Stefan},
  booktitle={24th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 15)},
  pages={897--912},
  year={2015}
}

@inproceedings{PrimeAbort,
  title={Prime+ abort: A timer-free high-precision l3 cache attack using intel $\{$TSX$\}$},
  author={Disselkoen, Craig and Kohlbrenner, David and Porter, Leo and Tullsen, Dean},
  booktitle={26th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 17)},
  pages={51--67},
  year={2017}
}

@inproceedings{CacheWebsiteFingerprinting,
  title={Robust website fingerprinting through the cache occupancy channel},
  author={Shusterman, Anatoly and Kang, Lachlan and Haskal, Yarden and Meltser, Yosef and Mittal, Prateek and Oren, Yossi and Yarom, Yuval},
  booktitle={28th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 19)},
  pages={639--656},
  year={2019}
}

@inproceedings{ReloadRefresh,
  title={Reload+ refresh: Abusing cache replacement policies to perform stealthy cache attacks},
  author={Briongos, Samira and Malag{\'o}n, Pedro and Moya, Jos{\'e} M and Eisenbarth, Thomas},
  booktitle={29th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 20)},
  year={2020}
}

@article{Pin,
  title={Pin: building customized program analysis tools with dynamic instrumentation},
  author={Luk, Chi-Keung and Cohn, Robert and Muth, Robert and Patil, Harish and Klauser, Artur and Lowney, Geoff and Wallace, Steven and Reddi, Vijay Janapa and Hazelwood, Kim},
  journal={Acm sigplan notices},
  volume={40},
  number={6},
  pages={190--200},
  year={2005},
  publisher={ACM New York, NY, USA}
}

@inproceedings{WeightedSpeedup,
  title={Symbiotic jobscheduling for a simultaneous multithreaded processor},
  author={Snavely, Allan and Tullsen, Dean M},
  booktitle={Proceedings of the ninth international conference on Architectural support for programming languages and operating systems},
  pages={234--244},
  year={2000}
}

@incollection{AlbonesiSerialTagData,
  title={An architectural and circuit-level approach to improving the energy efficiency of microprocessor memory structures},
  author={Albonesi, David H},
  booktitle={VLSI: Systems on a Chip},
  pages={192--205},
  year={2000},
  publisher={Springer}
}

@article{DEC,
  title={Internal organization of the Alpha 21164, a 300-MHz 64-bit quad-issue CMOS RISC microprocessor},
  author={Edmondson, John H. and Rubinfeld, Paul I. and Bannon, Peter J. and Benschneider, Bradley J. and Bernstein, Debra and Castelino, Ruben W. and Cooper, Elizabeth M. and Dever, Daniel E. and Donchin, Dale R. and Fischer, Timothy C. and others},
  journal={Digital Technical Journal},
  volume={7},
  number={1},
  year={1995}
}

@article{Itanium,
  title={The on-chip 3-mb subarray-based third-level cache on an itanium microprocessor},
  author={Weiss, Don and Wuu, John J and Chin, Victor},
  journal={IEEE Journal of Solid-State Circuits},
  volume={37},
  number={11},
  pages={1523--1529},
  year={2002},
  publisher={IEEE}
}

@inproceedings{IPDPS16_LLCPowerModel,
  title={A methodology for modeling dynamic and static power consumption for multicore processors},
  author={Goel, Bhavishya and McKee, Sally A},
  booktitle={2016 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},
  pages={273--282},
  year={2016},
  organization={IEEE}
}

@online{AnandTech_Power_Consumption,
    author = {AnandTech},
    title = {{Intel 9th Generation Power Consumption}},
    howpublished={\url{https://www.anandtech.com/show/13400/intel-9th-gen-core-i9-9900k-i7-9700k-i5-9600k-review/21}},
}

@inproceedings{PRINCE,
  title={{PRINCE--a low-latency block cipher for pervasive computing applications}},
  author={Borghoff, Julia and Canteaut, Anne and G{\"u}neysu, Tim and Kavun, Elif Bilge and Knezevic, Miroslav and Knudsen, Lars R and Leander, Gregor and Nikov, Ventzislav and Paar, Christof and Rechberger, Christian and others},
  booktitle={International conference on the theory and application of cryptology and information security},
  pages={208--225},
  year={2012},
  organization={Springer}
}


@online{PRINCE_vhdl,
    author = {Julian Harttung},
    title = {{PRINCE block cipher - VHDL implementation}},
    howpublished={\url{https://github.com/huljar/prince-vhdl}}
}

@inproceedings{15nmPDK,
  title={Open cell library in 15nm FreePDK technology},
  author={Martins, Mayler and Matos, Jody Maick and Ribas, Renato P and Reis, Andr{\'e} and Schlinker, Guilherme and Rech, Lucio and Michelsen, Jens},
  booktitle={Proceedings of the 2015 Symposium on International Symposium on Physical Design},
  pages={171--178},
  year={2015}
}

@inproceedings{Firesim,
  title={FireSim: FPGA-accelerated cycle-exact scale-out system simulation in the public cloud},
  author={Karandikar, Sagar and Mao, Howard and Kim, Donggyu and Biancolin, David and Amid, Alon and Lee, Dayeol and Pemberton, Nathan and Amaro, Emmanuel and Schmidt, Colin and Chopra, Aditya and others},
  booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)},
  pages={29--42},
  year={2018},
  organization={IEEE}
}

@inproceedings{FASED,
  title={FASED: FPGA-accelerated simulation and evaluation of DRAM},
  author={Biancolin, David and Karandikar, Sagar and Kim, Donggyu and Koenig, Jack and Waterman, Andrew and Bachrach, Jonathan and Asanovic, Krste},
  booktitle={Proceedings of the 2019 ACM/SIGDA International Symposium on Field-Programmable Gate Arrays},
  pages={330--339},
  year={2019}
}

@article{Gem5,
  title={The gem5 simulator},
  author={Binkert, Nathan and Beckmann, Bradford and Black, Gabriel and Reinhardt, Steven K and Saidi, Ali and Basu, Arkaprava and Hestness, Joel and Hower, Derek R and Krishna, Tushar and Sardashti, Somayeh and others},
  journal={ACM SIGARCH computer architecture news},
  volume={39},
  number={2},
  pages={1--7},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{BRUTUS,
  title={Brutus: Refuting the Security Claims of the Cache Timing Randomization Countermeasure Proposed in CEASER},
  author={Bodduna, Rahul and Ganesan, Vinod and SLPSK, Patanjali and Veezhinathan, Kamakoti and Rebeiro, Chester},
  journal={IEEE Computer Architecture Letters},
  volume={19},
  number={1},
  pages={9--12},
  year={2020},
  publisher={IEEE}
}

@phdthesis{MitzenmacherRealThesis, 
title={The Power of Two Choices in Randomized Load Balancing}, 
school={University of California at Berkeley},
author={Mitzenmacher, Michael}, 
year={1996},
howpublished={\url{http://eecs.harvard.edu/~michaelm/postscripts/mythesis.pdf}}}

@inproceedings{simpoints,
author = {Sherwood, Timothy and Perelman, Erez and Hamerly, Greg and Calder, Brad},
title = {Automatically Characterizing Large Scale Program Behavior},
year = {2002},
booktitle = {Proceedings of the 10th International Conference on Architectural Support for Programming Languages and Operating Systems},
series = {ASPLOS X}
}


